Mobile Energy Requirements of the Upcoming NIST Post-Quantum Cryptography Standards

Standardization of Post-Quantum Cryptography (PQC) was started by NIST in 2016 and has proceeded to its second elimination round. The upcoming standards are intended to replace (or supplement) current RSA and Elliptic Curve Cryptography (ECC) on all targets, including lightweight, embedded, and mobile systems. We present an energy requirement analysis based on extensive measurements of PQC candidate algorithms on a Cortex M4 - based reference platform. We relate computational (energy) costs of PQC algorithms to their data transmission costs which are expected to increase with new types of public keys and ciphertext messages. The energy, bandwidth, and latency needs of PQC algorithms span several orders of magnitude, which is substantial enough to impact battery life, user experience, and application protocol design. We propose metrics and guidelines for PQC algorithm usage in IoT and mobile systems based on our findings. Our evidence supports the view that fast structured-lattice PQC schemes are the preferred choice for cloud-connected mobile devices in most use cases, even when per-bit data transmission energy cost is relatively high.

==> Makefile <==
#	Makefile
#	2019-11-20	Markku-Juhani O. Saarinen <mjos@pqshield.com>

# main file
PROJ		= pqpstxt

# All latex source files
TEXFILES	= $(PROJ).tex avgpwr.tex results.tex crossover.tex

# Bibfile
BIBFILE		= pqcrypto.bib

# Uses xelatex for additional fonts
$(PROJ).pdf:	$(TEXFILES) $(BIBFILE)
		pdflatex $(PROJ)
		bibtex $(PROJ)
		pdflatex $(PROJ)
		pdflatex $(PROJ)

# sort the bibliography
#bibsort:
#		bibtool -s -r bibtool.cfg $(BIBFILE) > new_$(BIBFILE)

# clean does not remove the pdf file result
clean:
		rm -f	*.aux *.dvi *.bbl *.blg *.log *.toc *.lof \
			*.thm *.out $(PROJ)-*.tgz $(PROJ).pdf

dist:	clean
		cd ..; \
		tar cfvzh $(PROJ)/$(PROJ)-`date -u "+%Y%m%d%H%M"`.tgz \
			$(PROJ)/* $(PROJ)/.gitignore


